It might be balanced, but is it actually good? An Empirical Evaluation of Game Level Balancing

Achieving optimal balance in games is essential to their success, yet reliant on extensive manual work and playtesting. To facilitate this process, the Procedural Content Generation via Reinforcement Learning (PCGRL) framework has recently been effectively used to improve the balance of existing game levels. This approach, however, only assesses balance heuristically, neglecting actual human perception. For this reason, this work presents a survey to empirically evaluate the created content paired with human playtesting. Participants in four different scenarios are asked about their perception of changes made to the level both before and after balancing, and vice versa. Based on descriptive and statistical analysis, our findings indicate that the PCGRL-based balancing positively influences players' perceived balance for most scenarios, albeit with differences in aspects of the balancing between scenarios.

==> content/backup.tex <==
% SCENARIOS

\begin{figure}[htbp]
\centering
% SCENARIO 1
\begin{subfigure}[b]{0.4\textwidth}
\centering
   \begin{subfigure}[b]{0.46\textwidth}
    \includegraphics[width=\textwidth]{content/img/levels/WaterSwapUnbalancedGrid.png}
    \caption*{Unbalanced}
  \end{subfigure}
  \hspace{2mm}
   \begin{subfigure}[b]{0.46\textwidth}
    \includegraphics[width=\textwidth]{content/img/levels/WaterSwapBalancedGrid.png}
    \caption*{Balanced}
  \end{subfigure} 
  \vspace{-3mm}
 \caption{Scenario 1}
    \label{fig:s1}
  \end{subfigure}
\vspace{4mm}

% SCENARIO 2
 \begin{subfigure}[b]{0.4\textwidth}
 \centering
   \begin{subfigure}[b]{0.46\textwidth}
    \includegraphics[width=\textwidth]{content/img/levels/MountainBlockUnbalancedGrid.png}
    \caption*{Unbalanced}
  \end{subfigure}
  \hspace{2mm}
   \begin{subfigure}[b]{0.46\textwidth}
    \includegraphics[width=\textwidth]{content/img/levels/MountainBlockBalancedGrid.png}
    \caption*{Balanced}
  \end{subfigure} 
  \vspace{-3mm}
 \caption{Scenario 2}
    \label{fig:s2}
  \end{subfigure}
\vspace{4mm}

% SCENARIO 3
      \begin{subfigure}[b]{0.4\textwidth}
      \centering
   \begin{subfigure}[b]{0.46\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/levels/EqualizeLineUnbalancedGrid.png}
    \caption*{Unbalanced}
  \end{subfigure}
  \hspace{2mm}
   \begin{subfigure}[b]{0.46\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/levels/EqualizeLineBalancedGrid.png}
    \caption*{Balanced}
  \end{subfigure} 
  \vspace{-3mm}
 \caption{Scenario 3}
    \label{fig:s3}
  \end{subfigure}
  \vspace{4mm}
  
% SCENARIO 4
      \begin{subfigure}[b]{0.4\textwidth}
      \centering
   \begin{subfigure}[b]{0.46\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/levels/MountainBlock2BalancedGrid.png}
    \caption*{Balanced}
  \end{subfigure}
  \hspace{2mm}
   \begin{subfigure}[b]{0.46\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/levels/MountainBlock2UnbalancedGrid.png}
    \caption*{Unbalanced}
  \end{subfigure} 
  \vspace{-3mm}
 \caption{Scenario 4}
    \label{fig:s4}
  \end{subfigure}

\caption{The four scenarios included for playtesting. Levels in scenarios 1-3 were balanced from a previously unbalanced version. The balanced level in scenario 4 is the balanced version of scenario 2, which has was then further automatically unabalanced.}
\label{fig:scenarios}
\end{figure}


% This happens for 12.9\% of values $v$, either $v<-2$ or $v>2$.



% TABLE MEDIAN ONLY

\begin{table*}
    \centering
    \caption{Descriptive comparison of median values of unbalanced version (U) to balanced (B).}
    \begin{tabular}{lcccccccc} \toprule 
        & \multicolumn{2}{c}{Scenario 1} & \multicolumn{2}{c}{Scenario 2} & \multicolumn{2}{c}{Scenario 3} & \multicolumn{2}{c}{Scenario 4} \\
    
         \textbf{Item} &  \textbf{U}&  \textbf{B}&  \textbf{U}&\textbf{B} &  \textbf{U}&  \textbf{B}&  \textbf{B}&\textbf{U} \\         
         
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Movement Difficulty Player & 1& 1&    \textbf{-2}& \textbf{0}& 2& 2&   \textbf{-0.5}& \textbf{-1}\\
        Movement Difficulty Opponent & 1 & 1   & 2 & 2 & \textbf{1}& \textbf{2}&   \textbf{1}& \textbf{2}\\
        
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Amount Food Player & 0 & 0 &   \textbf{-1.5} & \textbf{1} & 1  & -1 & -1 & -1 \\
        Amount Food Opponent & \textbf{0}& \textbf{-1}&   2 & 2 &   0 & 0    & 2 & 2 \\
        
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Amount Water Player & \textbf{-1.5}& \textbf{0}&    0 & 0 &   0 & 0    & 0 & 0 \\
        Amount Water Opponent & 0.5 & 1 &    \textbf{1}& \textbf{0}& 1 & 1   & 0 & 0 \\   
                 
        
        \bottomrule
    \end{tabular}
    \label{tab:res-median}
\end{table*}


% TABLE WILCOXON ONLY

\begin{table*}
    \centering
    \caption{Results of the Wilcoxon signed-rank tests for each scenario per variable comparing the unbalanced with the balanced version. Significant values for $p \le 0.05$ are highlighted.}
    \begin{tabular}{lcccccccc} \toprule 
        & \multicolumn{2}{c}{Scenario 1} & \multicolumn{2}{c}{Scenario 2} & \multicolumn{2}{c}{Scenario 3} & \multicolumn{2}{c}{Scenario 4} \\
    
         \textbf{Item} &  \textbf{W}&  \textbf{p}&  \textbf{W}&\textbf{p}&  \textbf{W}&  \textbf{p}&  \textbf{W}&\textbf{p} \\         
         
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Movement Difficulty Player & 35 & 0.225 &  \textbf{5.5} & \textbf{0.00002} &  \textbf{4.5}& \textbf{0.034}& 15 & 0.357 \\
        Movement Difficulty Opponent & 20 & 0.740 &  \textbf{0} & \textbf{0.007} &  \textbf{0}& \textbf{0.005}& 6.5 & 0.190 \\
        
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Amount Food Player & 3 & 0.180 &  \textbf{7.5} & \textbf{0.0007} & 20 & 0.740 & 7 & 0.206 \\
        Amount Food Opponent & \textbf{4} & \textbf{0.035} &  3 & 1.0 & 12 & 0.705 & 2 & 0.564 \\
        
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        Amount Water Player & \textbf{10.5} & \textbf{0.007} &  \textbf{0.0} & \textbf{0.006} & 22.5 & 1.0 & 9 & 0.194 \\
        Amount Water Opponent & 19.5 & 0.083 &  \textbf{11} & \textbf{0.019} & 10.5 & 1.0 & 2 & 0.257 \\   
                 
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \morecmidrules
        \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        
        Samples & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{23} & \multicolumn{2}{c}{12} \\
        Critical Value for W & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{53} & \multicolumn{2}{c}{73} & \multicolumn{2}{c}{13} \\
        \bottomrule
    \end{tabular}
    \label{tab:res-wilcoxon}
\end{table*}
